Constraining the Black Hole Mass Spectrum with LISA Observations II: Direct comparison of detailed models

A number of scenarios have been proposed for the origin of the supermassive black holes (SMBHs) that are found in the centres of most galaxies. Many such scenarios predict a high-redshift population of massive black holes (MBHs), with masses in the range 100 to 100000 times that of the Sun. When the Laser Interferometer Space Antenna (LISA) is finally operational, it is likely that it will detect on the order of 100 of these MBH binaries as they merge. The differences between proposed population models produce appreciable effects in the portion of the population which is detectable by LISA, so it is likely that the LISA observations will allow us to place constraints on them. However, gravitational wave detectors such as LISA will not be able to detect all such mergers nor assign precise black hole parameters to the merger, due to weak gravitational wave signal strengths. This paper explores LISA's ability to distinguish between several MBH population models. In this way, we go beyond predicting a LISA observed population and consider the extent to which LISA observations could inform astrophysical modellers. The errors in LISA parameter estimation are applied with a direct method which generates random sample parameters for each source in a population realisation. We consider how the distinguishability varies depending on the choice of source parameters (1 or 2 parameters chosen from masses, redshift or spins) used to characterise the model distributions, with confidence levels determined by 1 and 2-dimensional tests based on the Kolmogorov-Smirnov test.

==> figures/LISA_Quadplot2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(8640.00,6048.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1188,823){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1188,1557){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1188,2290){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1188,3023){\makebox(0,0)[r]{\strut{} 100}}%
      \put(2000,220){\makebox(0,0){\strut{} 5}}%
      \put(2800,220){\makebox(0,0){\strut{} 10}}%
      \put(3600,220){\makebox(0,0){\strut{} 15}}%
      \put(418,1731){\rotatebox{90}{\makebox(0,0){\strut{}dN/dzdt [1/yr]}}}%
      \put(2820,-110){\makebox(0,0){\strut{}detected redshift $z_d$}}%
      \put(1480,2802){\makebox(0,0)[l]{\strut{}$10^4 M_\odot<M_{BH}<10^6 M_\odot$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4188,823){\makebox(0,0)[r]{\strut{}}}%
      \put(4188,1557){\makebox(0,0)[r]{\strut{}}}%
      \put(4188,2290){\makebox(0,0)[r]{\strut{}}}%
      \put(4188,3023){\makebox(0,0)[r]{\strut{}}}%
      \put(5000,220){\makebox(0,0){\strut{} 5}}%
      \put(5800,220){\makebox(0,0){\strut{} 10}}%
      \put(6600,220){\makebox(0,0){\strut{} 15}}%
      \put(5820,-110){\makebox(0,0){\strut{}detected redshift $z_d$}}%
      \put(4480,2802){\makebox(0,0)[l]{\strut{}$M_{BH}>10^6 M_\odot$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4188,3440){\makebox(0,0)[r]{\strut{}}}%
      \put(4188,4236){\makebox(0,0)[r]{\strut{}}}%
      \put(4188,5031){\makebox(0,0)[r]{\strut{}}}%
      \put(4188,5827){\makebox(0,0)[r]{\strut{}}}%
      \put(5000,2804){\makebox(0,0){\strut{}}}%
      \put(5800,2804){\makebox(0,0){\strut{}}}%
      \put(6600,2804){\makebox(0,0){\strut{}}}%
      \put(4480,5587){\makebox(0,0)[l]{\strut{}$M_{BH}<10^4 M_\odot$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \put(1188,3440){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(1188,4236){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1188,5031){\makebox(0,0)[r]{\strut{} 10}}%
      \put(1188,5827){\makebox(0,0)[r]{\strut{} 100}}%
      \put(2000,2804){\makebox(0,0){\strut{}}}%
      \put(2800,2804){\makebox(0,0){\strut{}}}%
      \put(3600,2804){\makebox(0,0){\strut{}}}%
      \put(418,4425){\rotatebox{90}{\makebox(0,0){\strut{}dN/dzdt [1/yr]}}}%
      \put(1480,5587){\makebox(0,0)[l]{\strut{}all BHs}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figures/LISA_Quadplot2_pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup

